Formal Analysis of Robotic Cell Injection Systems using Theorem Proving

Cell injection is an approach used for the delivery of small sample substances into a biological cell and is widely used in drug development, gene injection, intracytoplasmic sperm injection (ICSI) and in-virto fertilization (IVF). Robotic cell injection systems provide the automation of the process as opposed to the manual and semi-automated cell injection systems, which require expert operators and involve time consuming processes and also have lower success rates. The automation of the cell injection process is achieved by controlling the injection force and planning the motion of the injection pipette. Traditionally, these systems are analyzed using paper-and-pencil proof and computer simulation methods. However, the former is human-error prone and the later is based on the numerical algorithms, where the approximation of the mathematical expressions introduces inaccuracies in the analysis. Formal methods can overcome these limitations and thus provide an accurate analysis of the cell injection systems. Model checking, i.e., a state-based formal method, has been recently proposed for the analysis of these systems. However, it involves the discretization of the differential equations that are used for modeling the dynamics of the system and thus compromises on the completeness of the analysis of these safety-critical systems. In this paper, we propose to use higher-order-logic theorem proving, a deductive-reasoning based formal method, for the modeling and analysis of the dynamical behaviour of the robotic cell injection systems. The proposed analysis, based on the HOL Light theorem prover, enabled us to identify some discrepancies in the simulation and model checking based analysis of the same robotic cell injection system.

==> hol_macros.tex <==
%-------------------------------------------
%
% HOL Macros.
% Jim Alves-Foss (foss@iris.eecs.ucdavis.edu) [128.120.57.20]
% BETA VERSION November 1990
%
% Thanks to Tom Schubert, Jim Buffenbarger, and Phil Windley for
%   their help and contributions (directly or indirectly)
%
% This file consists of a collection of definitions and macros
% for use in LaTeX documents discussing the HOL language and
% its associated proofs.
%
% The primary macros introduced here are given below.
%
% NOTE: for holdef and holthm you must replace ALL lambda symbols
% `\' by `\. ' this can be accomplished automatically in HOL by the command:
%   set_lambda`\\.`;;
% Which will then display the lamda symbol as`\. ' but will permit input to
% still be `\'.
%
% \holthm{defn}  Which takes defn (cut directly from HOL output
%                and converts all the symbols (ie. |- ==>) to their
%                mathematical equivalents.
%
% \holdef{defn}  Same as holthm except that the turnstile is subscripted
%                by ``def''
%
% \begin{hol} ... \end{hol} Defines an environment for HOL theorems and
%                definitions. This environment it identical to alltt except
%                that it places a box around the text and ~ still works
%
% \begin{holnb} ... \end{holnb} Same as ``hol'' but no box
%
% and you must include this file:
% \include{hol_macros}
%
%-------------------------------------------


% HOLTT DOCUMENT-STYLE OPTION -
% Modified for HOL macro use Nov 1990 by Jim Alves-Foss and Phil Windley from :

% ALLTT DOCUMENT-STYLE OPTION - released 17 December 1987
%    for LaTeX version 2.09
% Copyright (C) 1987 by Leslie Lamport


% Defines the `alltt' environment, which is like the `verbatim'
% environment except that `\', `\{', and `\}' have their usual meanings.
% Thus, other commands and environemnts can appear within an `alltt'
% environment.  Here are some things you may want to do in an `alltt'
% environment:
%
% * Change fonts--e.g., by typing `{\em empasized text\/}'.
%
% * Insert text from a file foo.tex by typing `input{foo}'.  Beware that
%   each <return> stars a new line, so if foo.tex ends with a <return>
%   you can wind up with an extra blank line if you're not careful.
%
% * Insert a math formula.  Note that `$' just produces a dollar sign,
%   so you'll have to type `\(...\)' or `\[...\]'.  Also, `^' and `_'
%   just produce their characters; use `\sp' or `\sb' for super- and
%   subscripts, as in `\(x\sp{2}\)'.


\makeatletter

\def\holdocspecials{\do\ \do\$\do\&%
  \do\#\do\^\do\^^K\do\_\do\^^A\do\%}

\def\holtt{\trivlist \item[]\if@minipage\else\vskip\parskip\fi
\leftskip\@totalleftmargin\rightskip\z@
\parindent\z@\parfillskip\@flushglue\parskip\z@
\@tempswafalse \def\par{\if@tempswa\hbox{}\fi\@tempswatrue\@@par}
%\obeylines \tt \catcode``=13 \@noligs \let\do\@makeother \holdocspecials
\obeylines \tt \let\do\@makeother \holdocspecials
 \frenchspacing\@vobeyspaces}

\let\endholtt=\endtrivlist

\makeatother

\newlength{\hsbw}
\setlength{\hsbw}{\textwidth}
\addtolength{\hsbw}{-\arrayrulewidth}
\addtolength{\hsbw}{-\tabcolsep}
\newcommand\HOLSpacing{13pt}

% ---------------------------------------------------------------------
% Macro for boxed ML functions, etc.
%
% Usage: (1) \begin{boxed}\begin{verbatim}
%	        .
%	        < lines giving names and types of mk functions >
%	        .
%	     \end{verbatim}\end{boxed}
%
%            typesets the given lines in a box.
%
%            Conventions: lines are left-aligned under the "g" of begin,
%	     and used to highlight primary reference for the ml function(s)
%	     that appear in the box.
% ---------------------------------------------------------------------

\renewenvironment{boxed}{\begin{flushleft}
 \begin{tabular}{@{}|c@{}|@{}}\hline
 \begin{minipage}[b]{\hsbw}
 \vspace*{.06in}
 \begingroup\small\baselineskip\HOLSpacing}{\endgroup\end{minipage}\\ \hline
 \end{tabular}
 \end{flushleft}}

\newenvironment{hol}{\begin{flushleft}
 \begin{tabular}{@{}|c@{}|@{}}\hline
 \begin{minipage}[b]{\hsbw}
 \vspace*{.06in}
 \begingroup\small\baselineskip\HOLSpacing\footnotesize
 \begin{holtt}}{\end{holtt}\endgroup
 \end{minipage}\\ \hline
 \end{tabular}
 \end{flushleft}}

% HOL environment not boxed %
\newenvironment{holnb}{\begin{flushleft}
 \begin{minipage}[b]{\hsbw}
 \vspace*{.02in}
 \begingroup\small\baselineskip\HOLSpacing\footnotesize
 \begin{holtt}}{\end{holtt}\endgroup
 \end{minipage}
 \end{flushleft}}

   \newcommand\hilbert{\varepsilon}
   \newcommand{\Defn}{\(\vdash\sb{\it def}\)}
   \newcommand{\Thm}{\(\vdash\)}
   \newcommand{\Cond}{\(\Longrightarrow\)}
   \newcommand{\Eqv}{\(\equiv\)}
   \newcommand{\Iff}{\(\Leftrightarrow\)}
   \newcommand{\Fa}{\(\scriptsize \forall\)}
   \newcommand{\Et}{\(\exists\)}
   \newcommand{\Eu}{\(\exists_{unique}\)}
   \newcommand{\La}{\(\land\)}
   \newcommand{\Lo}{\(\lor\)}
   \newcommand{\Lx}{\(\oplus\)}
   \newcommand{\Lc}{\(\lnot\)}
   \newcommand{\Impl}{\(\Longrightarrow\)}
   \newcommand{\Func}{\(\to\)}
   \renewcommand{\Bar}{\(\mid\)}
   \newcommand{\uqu}[1]{\(\forall\)\ #1.\ }
   \newcommand{\equ}[1]{\(\exists\)\ #1.\ }
   \newcommand{\hqu}[1]{\(\hilbert\)\ #1.\ }
   \newcommand{\lqu}[1]{\(\lambda\)\ #1.\ }
   \newcommand{\Lam}{\(\lambda\)}
   \newcommand{\Plus}{\(+\)}
   \newcommand{\Minus}{\(-\)}
   \newcommand{\Prime}{\('\)}
   \newcommand{\Und}{\_}
   \newcommand{\Lt}{\(<\)}
   \newcommand{\Gt}{\(>\)}
   \newcommand{\Leq}{\(\leq\)}
   \newcommand{\Geq}{\(\geq\)}
   \newcommand{\Eq}{\(=\)}

\newcommand{\Hilbert}{\(\hilbert\)}
\newcommand{\Imp}{\(\Rightarrow\)}
\newcommand{\Conj}{\(\wedge\)}
\newcommand{\Disj}{\(\vee\)}
\newcommand{\Neg}{\(\neg\)}
\newcommand{\Pnd}{\(\Diamond\)}
\newcommand{\var}[1]{{\it #1}}

%----------------
%  The following are recursive definitions that take HOL output and convert
%  it into a nice mathematical format in LaTeX. Use holthm for theorems and
%  holdef for definitions (Warning do not include too many definitions or
%  theorems together, as the TeX buffer will overflow
%---------------

\long\def\holthm#1{{\def\Turns{\Thm} \rechol#1\end\end\end}}

\long\def\holdef#1{{\def\Turns{\Defn} \rechol#1\end\end\end}}

\long\def\rechol#1#2#3{\let\next=\rechol\def\postnext{#2#3}\ifx#1\end
\let\next=\relax\def\postnext{\relax}
\else\ifx#1!\Fa                                          % For all !
\else\ifx#1@\Hilbert                                     % Hilbert Choice @
\else\ifx#1\#\Pnd                                        % Product #
\else\ifx#1'\Prime                                       % Prime  '
\else\ifx#1~\Neg                                         % Negation  ~
\else\ifx#1\~\Neg
\else\ifx#1_\Und                                         % Underscore  _
\else\ifx#1+\Plus
\else\ifx#1\/\Disj                                       % Disjunction  \/
\else\ifx#1\.\Lam                                        % Remove cntrl seq
\else\ifx#1>\ifx#2=\Geq\def\postnext{#3}\else\Gt\fi      % Greater, Geq >  >=
\else\ifx#1?\ifx#2!\Eu\def\postnext{#3}\else\Et\fi       % Exists(unique) ? ?!
\else\ifx#1-\ifx#2\>\Func\def\postnext{#3}               % Minus, Function
	    \else\Minus\fi				 % - ->
\else\ifx#1|\ifx#2-\Turns\def\postnext{#3}\else\Bar\fi   % Turnstile,Bar |- |
\else\ifx#1<\ifx#2=\ifx#3>\Iff\def\postnext{}            % Less, Leq, Iff
                   \else\Leq\def\postnext{#3}\fi         % <  <=  <=>
            \else\Lt\fi
\else\ifx#1=\ifx#2=\ifx#3>\Imp\def\postnext{}            % Eq, Eqv, Cond, Imp
                   \else\Eqv\def\postnext{#3}\fi         % = == => ==>
            \else\ifx#2>\Cond\def\postnext{#3}
                 \else\Eq\fi\fi
\else\ifx#1/\ifx#2\^^M\Conj\par\def\postnext{#3}         % Conjunction, slash
            \else\ifx#2\ \Conj\ \def\postnext{#3}\else#1\fi\fi  % /\  /
\else#1\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\expandafter\next\postnext}







